Learning to Simulate Individuals from Macro Social Signals

Large language models are increasingly used to simulate how individuals respond to new situations, yet the behavioral reasoning behind these responses is either inherited from pretraining or learned from individual-level annotations, which offer limited behavioral diversity and little supervision of the reasoning itself. We propose to learn behavioral reasoning from prediction markets, whose price trajectories record how populations respond to real-world events at scale. We introduce macro2mind, which trains a language model with GRPO using market signals. A social behavioral decomposition makes behavioral reasoning an explicit step of forecasting: the model infers representative groups of market participants, predicts how each interprets the news and updates its beliefs, reasons about their interactions, and aggregates these responses into a price. A hindsight-regret curriculum with difficulty-aware sampling focuses training on transitions where hindsight-identified groups substantially improve the forecast while prioritizing examples that remain learnable for the current policy. The learned reasoning applies to user simulation without further training. On SWM-Bench, macro2mind achieves state-of-the-art directional accuracy and correlation on Polymarket. Trained on market data, it transfers zero-shot to four user-simulation benchmarks (Humanual, OvertonBench, PRISM, and CAD) and has competitive performance among zero-shot methods. Used as a data generator, macro2mind also raises a downstream simulator's accuracy on unseen users by 15.5 points, outperforming data generated by its backbone by 13.2 points.

==> tables/user_sim_ori.tex <==
\begin{table}[t]
\centering
\caption{
User simulation performance.
State Align. and Response Align. denote state and response
alignment on Humanual-Politics.
OvertonBench results use the \texttt{fs+fr} condition.
PRISM MAE is reported on the original rating scale, and
pairwise preference accuracy is reported as a percentage.
}
\label{tab:user_simulation}
\small
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1}
\label{tab:user_simulation}
\small
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1}
\begin{tabular*}{\linewidth}{
    @{\extracolsep{\fill}} l c c c c c c c @{}
}
\toprule
& \multicolumn{2}{c}{Humanual-Politics}
& \multicolumn{2}{c}{OvertonBench}
& \multicolumn{2}{c}{PRISM}
& \multicolumn{1}{c}{CAD} \\
\cmidrule(lr){2-3}
\cmidrule(lr){4-5}
\cmidrule(lr){6-7}
\cmidrule(lr){8-8}
Model
& State Align. $\uparrow$
& Response Align. $\uparrow$
& MAE $\downarrow$
& Spearman $\rho$ $\uparrow$
& MAE $\downarrow$
& Pairwise Acc. (\%) $\uparrow$
& Acc. (\%) $\uparrow$ \\
\midrule
Qwen3-4B (base)
& 0.077 & 0.024 & 0.756 & 0.539 & 21.46 & 62.4 & 38.9 \\
% Qwen3.8-Max
% & \textbf{0.133} & 0.045 & 0.673 & \textbf{0.693} & 23.66 & \textbf{67.2} & \textbf{42.2} \\
GRPO (4B)
& 0.061 & 0.015 & \textbf{0.623} & 0.647 & 22.99 & 53.9 & 36.6 \\
\textbf{Ours (4B)}
& 0.093 & 0.034 & 0.635 & \textbf{0.653} & \textbf{21.21} & 63.3 & 42.2 \\
\midrule
\multicolumn{8}{l}{\textit{Prompting-based (no fine-tuning)}} \\
Qwen3-4B                              & 0.077 & 0.024 & 0.756 & 0.539 & 21.5 & 62.4 & 38.9 \\
Qwen3.8-Max                           & 0.133 & 0.045 & 0.673 & 0.693 & 23.7 & 67.2 & 42.2 \\
PERSONA-Flow                          & 0.075 & 0.021 & 0.756 & 0.540 & 21.5 & 62.5 & 38.8 \\
Qwen3-4B + History-ICL                & 0.088 & 0.029 & 0.741 & 0.552 & 20.5 & 63.6 & 42.9 \\
Qwen3-4B + SynthesizeMe               & 0.077 & 0.022 & 0.763 & 0.529 & 21.3 & 63.2 & 40.4 \\
Qwen3-4B + Self-report                & 0.069 & 0.018 & 0.750 & 0.544 & 21.5 & 62.7 & 38.5 \\
Qwen3-4B + Self-consistency ($n{=}5$) & 0.079 & 0.021 & 0.758 & 0.538 & 21.3 & 62.6 & 38.6 \\
\midrule
\multicolumn{8}{l}{\textit{Training-based (fine-tuned; training data in parentheses)}} \\
GRPO {\scriptsize (SWMBench)}              & 0.061 & 0.015 & 0.623 & 0.647 & 23.0 & 53.9 & 36.6 \\
HumanLM-SFT {\scriptsize (Humanual)}       & 0.082$^\ddagger$ & 0.032$^\ddagger$ & 0.734 & 0.566 & 22.5 & 59.6 & 35.0 \\
HumanLM-SFT-think {\scriptsize (Humanual)} & 0.063$^\ddagger$ & 0.018$^\ddagger$ & 0.754 & 0.606 & 23.3 & 60.1 & 36.5 \\
HumanLM-GRPO {\scriptsize (Humanual)}      & 0.124$^\ddagger$ & 0.053$^\ddagger$ & 0.718 & 0.576 & 21.8 & 62.6 & 39.1 \\
P-GenRM {\scriptsize (PRISM)}              & 0.034 & 0.007 & 0.786 & 0.455 & 21.8$^{\ddagger\dagger}$ & 66.2$^{\ddagger\dagger}$ & 44.0 \\
Skywork-RM {\scriptsize (pretrained)}      & 0.083 & 0.024 & 1.024 & 0.090 & 21.5   & 64.7 & 41.8 \\
MRM {\scriptsize (per benchmark)}          & 0.078$^\ddagger$ & 0.025$^\ddagger$ & 0.907$^\ddagger$ & 0.338$^\ddagger$ & 20.7 & 69.1$^{\ddagger\dagger}$ & 44.2$^\ddagger$ \\
WIMHF-RM {\scriptsize (per benchmark)}     & 0.079$^\ddagger$ & 0.026$^\ddagger$ & 0.859$^\ddagger$ & 0.429$^\ddagger$ & 20.7 & 69.5$^{\ddagger\dagger}$ & 43.6$^\ddagger$ \\


% Unless marked, cells are zero-shot: the model was trained only on the data in parentheses
% (Ours: SWMBench). Generative simulators follow their original single-source setting
% (HumanLM: Humanual; P-GenRM: PRISM) and are not re-tuned per benchmark, which would give
% them in-domain supervision that Ours does not receive.
% $^\ddagger$ In-domain: the model was trained on that benchmark's training data.
% Scalar reward models (MRM, WIMHF-RM) cannot be transferred zero-shot (e.g.\ reward-to-rating
% calibration on Overton collapses to a constant, $\rho\approx0.09$ for Skywork-RM), so, following
% their original per-dataset setting, one model is trained per benchmark; these cells are in-domain
% and are reported for reference, not as a like-for-like comparison.
% For reward models, Humanual cells rerank 8 sampled Qwen3-4B candidates (T{=}0.7) and judge the
% top one (uniform pick: 0.076 / 0.022); Overton maps the reward to 1--5 by isotonic regression.
% $^\dagger$ Training and test turns overlap on PRISM (unseen-turn Pairwise Acc.: MRM 68.6, WIMHF-RM 68.8). \\
% For reward models, rating columns (Overton, PRISM MAE) map the reward to the rating scale by
% isotonic regression fit on held-out gold ratings (PRISM: 5-fold cross-fitting grouped by user);
% $^{\S}$ this calibration uses PRISM labels, so Skywork-RM's PRISM MAE is not strictly zero-shot..


% ======================================================================
% Baseline 说明（Table 1: user simulation；strict 口径）
% 口径：未解析一律按失败计入——Humanual 未解析记 0；Overton 未解析记 3；
%   PRISM 未解析的 turn 记 50，且它参与的所有成对比较都算排错；
%   CAD 未解析算选错。CAD 用 2000 行英文子集；Overton 用 political 子划分，
%   fs+fr 共 7200 行；PRISM 测试集 = study 全部 27,172 个 turn。
%   Humanual 由 qwen3.8-max 作 judge。
% 结果台账（权威）：/home/yiningz9/lbs/bl/RESULTS_LEDGER_20260923.md
% 代码仓库（worktree）：/home/yiningz9/lbs/bl/swm_rl_baselines
%   （GitHub: negativegluon/swm_rl_new，脚本在 scripts/baselines/）
% 远程结果本机副本：/home/yiningz9/lbs/bl/remote_results
% ----------------------------------------------------------------------
% [Ours] cotrl-belief-ep03-regret。
%   ckpt: /home/yiningz9/lbs/bl/twin_synthetic_sft_ckpt/teachers/cotrl-belief-ep3-regret
%
% ---- Prompting-based（不微调）----
% Qwen3-4B / Qwen3.8-Max：直接提示做用户模拟（Qwen3, arXiv 2505.09388）。
%   Qwen3.8-Max 通过 DashScope API 调用；Qwen3-4B 用本地 vLLM 推理。
% PERSONA-Flow：PERSONA (arXiv 2602.15669) 的 persona-vector 引导方法，
%   基座为 Qwen3-4B。脚本 scripts/baselines/persona_flow_fill.py、
%   run_parallel_fill_eval.sh；persona 向量在 third_party/persona/。
% +History-ICL：用 BM25 检索该用户的历史作 in-context 示例（本文实现的通用基线）。
% +SynthesizeMe：先从用户历史归纳出 persona，再做模拟（arXiv 2506.05598）。
% +Self-report：让模型以第一人称自述"我是谁/我怎么看"，再作答（本文实现）。
% +Self-consistency(n=5)：采样 5 次后投票/取平均（Wang et al., arXiv 2203.11171）。
%   以上 4 种：scripts/baselines/prompt_methods.py、
%   run_parallel_prompting_eval.sh、tests/test_prompt_methods.py；
%   方法调研报告：/home/yiningz9/lbs/bl/prompting_baselines_survey.md
%   （参考 SimBench, arXiv 2510.17516）。
%
% ---- Training-based（括号内为训练数据；其余 benchmark 均为 zero-shot 迁移）----
% GRPO (SWMBench)：即 freerl 实验（ffrl-base），在 SWMBench 上做 GRPO
%   (DeepSeekMath, arXiv 2402.03300)；与 Ours 同一套训练框架。
% HumanLM-SFT / -SFT-think / -GRPO (Humanual)：HumanLM 论文 (arXiv 2603.03303)
%   的训练配方，基座 Qwen3-4B，在 Humanual train 上训练。
%   -SFT-think 带思考过程；-GRPO 只训到第 50 步（共 354 步）。
%   HumanLM 论文的主方法本身没有复现，只复现了它的 SFT/GRPO 配方。
%   评测脚本：scripts/baselines/run_server_humanlm.sh、run_parallel_humanlm_eval.sh、
%   run_parallel_any_eval.sh；奖励 shim：humanlm_reward_shim.py。
% P-GenRM (PRISM)：生成式个性化奖励模型 (arXiv 2602.12116)，在 PRISM 上训练；
%   表中用 stage3，并把它当作生成式模拟器跑全部 4 个 benchmark。
%   PRISM 列与训练集有重叠（†）。
%   脚本：scripts/baselines/pgenrm_shard_launch.py、run_parallel_pgenrm_infer.sh。
%   推理用 4096 tokens 生成上限 / 10240 上下文窗口，未解析的行补跑；
%   Humanual 上约 24% 的回复被截断。
% Skywork-RM (pretrained)：Skywork-Reward V1/V2 通用标量奖励模型，不做任何训练。
% MRM (per benchmark)：元学习个性化奖励模型 (arXiv 2601.18731)：在 Skywork
%   embedding 上元训练一个 MLP，评测时对每个用户做 leave-one-conversation-out 适配。
% WIMHF-RM (per benchmark)：WIMHF (ICLR 2026)：Qwen3-4B LoRA 奖励模型 + SAE 特征。
% 标量 RM 的迁移方式：
%   CAD 对 4 个选项打分取 argmax；PRISM 按奖励分排序算 pairwise；
%   Overton 用 isotonic 把奖励映射到 1-5 后取整；
%   Humanual 对 8 个 Qwen3-4B 候选回复做 best-of-8 重排后交 judge 打分；
%   PRISM MAE 不适用（--）。
%   "per benchmark" = 每个 benchmark 单独训一个（PRISM 用官方发布的模型，
%   有训练重叠 †；只看训练外 turn：MRM 68.6，WIMHF 68.8）。
%   零样本迁移：scripts/baselines/rm_eval_tool.py、run_parallel_rm_eval.sh
%     → outputs/baselines/rm_eval/{RESULTS.txt,metrics.json}
%   分 benchmark 训练：scripts/baselines/rm_train_tool.py、run_local_rm_train_eval.sh
%     → outputs/baselines/rm_train/{results/RESULTS.txt,metrics.json,wimhf/,mrm/}
%   （以上路径相对 /home/yiningz9/lbs/bl/swm_rl_baselines；
%     rm_* 脚本当前尚未 push 到 GitHub。）
%
% ---- Benchmark 出处 ----
% Humanual：随 HumanLM 发布 (arXiv 2603.03303)；
% OvertonBench (arXiv 2512.01351, ICLR 2026)；PRISM (arXiv 2404.16019)；
% CAD = Community Alignment (arXiv 2507.09650)。
% ======================================================================

%有问题可以删掉任意的



\bottomrule
\end{tabular*}
\end{table}

